Unsupervised Representation Disentanglement of Text: An Evaluation on Synthetic Datasets

To highlight the challenges of achieving representation disentanglement for text domain in an unsupervised setting, in this paper we select a representative set of successfully applied models from the image domain. We evaluate these models on 6 disentanglement metrics, as well as on downstream classification tasks and homotopy. To facilitate the evaluation, we propose two synthetic datasets with known generative factors. Our experiments highlight the existing gap in the text domain and illustrate that certain elements such as representation sparsity (as an inductive bias), or representation coupling with the decoder could impact disentanglement. To the best of our knowledge, our work is the first attempt on the intersection of unsupervised representation disentanglement and text, and provides the experimental framework and datasets for examining future developments in this direction.

==> backup/disentanglement.tex <==
%\ehsan{connect to human intelligence}
%Although studying representation disentanglement in VAEs including encouraging \citep{pmlr-v80-kim18b,burgess2018,higgins2016}, understanding \citep{pmlr-v97-mathieu19a,burgess2018} as well as evaluating \citep{Chen2018isolating,eastwood2018a,pmlr-v80-kim18b,higgins2016} is a common practice in image domain, minor works, to the best of our knowledge, focus on representation disentanglement for text.

%Disentanglement literature in VAEs for text mainly aim to split the latent space into two predefined disentangled subspace such as style and content space \citep{cheng-etal-2020-improving,john-etal-2019-disentangled}, or syntactic and semantic space \citep{bao-etal-2019-generating}. Their works are quite different than disentanglement literature for image where they hope to disentangle un-predefined single latent variables. In addition, these explorations require prior knowledge about datasets as well as some supervision during training, which is different from our goal to learn disentangled representations in a pure unsupervised setting. 

%An exception \citep{DBLP:journals/corr/abs-2012-13031} tries to disentangle semantics in sentences via pure unsupervised method, but this work does not give a disentanglement score to evaluate methods' ability in achieving disentanglement and make it difficult to compare different models. In our work, we propose two synthetic datasets to facilitate disentanglement score calculation via six different disentanglement metrics.
